Efficient and Versatile Robust Fine-Tuning of Zero-shot Models

Large-scale image-text pre-trained models enable zero-shot classification and provide consistent accuracy across various data distributions. Nonetheless, optimizing these models in downstream tasks typically requires fine-tuning, which reduces generalization to out-of-distribution (OOD) data and demands extensive computational resources. We introduce Robust Adapter (R-Adapter), a novel method for fine-tuning zero-shot models to downstream tasks while simultaneously addressing both these issues. Our method integrates lightweight modules into the pre-trained model and employs novel self-ensemble techniques to boost OOD robustness and reduce storage expenses substantially. Furthermore, we propose MPM-NCE loss designed for fine-tuning on vision-language downstream tasks. It ensures precise alignment of multiple image-text pairs and discriminative feature learning. By extending the benchmark for robust fine-tuning beyond classification to include diverse tasks such as cross-modal retrieval and open vocabulary segmentation, we demonstrate the broad applicability of R-Adapter. Our extensive experiments demonstrate that R-Adapter achieves state-of-the-art performance across a diverse set of tasks, tuning only 13% of the parameters of the CLIP encoders.

==> Sections/_1_intro_backup.tex <==
\section{Introduction}
\label{sec:intro}

% - CLIP이나 ALIGN과 같은 image와 text로 pretrained된 large-scale model들의 등장
% - 이들은 놀라울 만큼 다양한 data distribution에서 robust하게 reasonable한 zero-shot performance를 보여주고 있다.
% - 이러한 모델은 fine-tuning을 통해서 target task에서 더욱 크게 성능을 끌어올릴 수 있으나, 허나  [...]에서 관찰된 바와 같이 out-of-distribution data에서의 generalization ability가 감소하게된다.
% - 이러한 문제를 막기 위해서 여러가지 [...] 방법들이 제안 되었으나, 기존의 방법들은 모델 전체를 fine-tuning 방법들이기에, 모델이 크면  memory 및 computational overhead가 크게 증가하게 된다.
% - 이 paper에서는, 이러한 문제를 address하기 위하여 parameter-efficient learning한 학습 법에 대해서 다루려고 함.  Parameter efficient 방법은 pre-trained 모델에 적은 수의 새로운 parameter만을 사용하여 adapt하기 떄문에, catastropic forgetting을 막는것으로 알려져 있음. 허나 in practie에서 점차 학습하면서 adapt된 module들이 indistribution에 bias되면서 distribution shift에 완벽하게 대응하지는 못한다는 것을 observe함.  실제 실험결과들 Figure ... 
% -  이러한 문제를 막기 위하여, 우리는 Parameter-efficient Robust Finetuning (PERFT)를 제안함. PEFT는 efficient하면서도 OOD generalization ability를 향상시키는 effective한 방법이다. 
% - PERFT는 adapter ... 모듈 구조를 따르며, indistribution data를 통해 target task에 대한 information은 배우되, in-distribution에 bias되지 않게 제약 하는 3가지 전략을 사용한다. 우선, 우리는 [...]와 같이 ensemble이 accuracy와 robustness를 향상 시킬 수 있다는 관찰에 힘입어 stochastic drop 및 exponential moving average의 2가지 self-ensemble 전략을 채택한다. 그리고 핵심적으로, adapter의 output의 scale을 evaluation time에 rescaling하는 trick을 통해 bias의 overwhelming을 확실하게 통제한다.  한편, 우리의 adapter는 re-parametrization trick을 통해서 기존 모델 대비 additional한 computation을 추가하지 않는다.
% - 또한, 우리는 multimodal contrastive learning의 standard loss인 infoNCE 기반의 contrastive loss를 revisit하여, robust finetuning 위해 이를 개선한다.  기존의 loss는 따로 label을 고려하지 않고 sample 자신의 것 외의 pair 들을 모두 밀어버린다. 허나, 이는 기존 embedding space의 큰 변경을 가져오며, 이로 인해 robustness를 잃어버린다. 따라서 우리는, target task의 label에 기반하여 anchor에 대한 positive를 고려하면서, target task에서 가장 잘못 위치되어있는 hardnest negative sample만을 밀어낸다. 이는 결과적으로, embedding space의 최소한의 변화만을 가하면서도 target task를 위한 최적의 embedding space를 만들게된다.

\begin{figure} [!t]
\vspace{-3mm}
\centering
\includegraphics[width = 1.0\linewidth]{figs/Figure_thumbnail2.pdf}
\vspace{-7mm}
\caption{Comparative analysis of performance versus memory usage among robust fine-tuning methods. Memory usage is measured on an NVIDIA 3090 GPU at a batch size of 16. Our method utilizes less memory, which supports easily scaling up to larger models and broader applications, unlike most other methods.} 
\label{fig:thumbnail}
\vspace{-6mm}
\end{figure}

The emergence of large-scale models pre-trained jointly on image and text data, such as CLIP~\cite{clip}, brings a paradigm shift in the field of computer vision. The models leverage the power of contrastive learning to align vast collections of image-text pairs sourced from the web, enabling them to capture intricate relations between these two modalities. This training enables them to perform zero-shot classification, where previously unseen images are classified by comparing their embeddings with textual class descriptions. Impressively, these models show notable zero-shot performance across a wide range of data distributions.

While their performance is impressive in a zero-shot context, it still does not measure up to supervised models.
% To unlock their full potential for downstream tasks, fine-tuning is commonly applied, leading to substantial performance gains on the target in-distribution. Nevertheless, a noteworthy challenge arises from fine-tuning, as it diminishes their capacity to generalize to out-of-distribution (OOD) data~\cite{radford2021learning, jia2021scaling, pham2023combined, kumar2022fine}.
% This decrease in adaptability raises concerns, especially when considering the deployment of these models in real-world settings with unpredictable data variances.
To unlock their full potential for downstream tasks, fine-tuning is fine-tuning is often necessary. This boosts their performance significantly on the target distribution. Yet, a significant challenge emerges: traditional fine-tuning diminishes their capacity to generalize to out-of-distribution (OOD) data~\cite{clip, scalingshifting, pham2023combined, lpft}. This decrease in adaptability raises concerns, especially when considering the deployment of these models in real-world settings with unpredictable data variances.

% To mitigate these problems, several approaches have been proposed to fine-tune zero-shot models while preserving their robustness. These methods include strategies such as ensembling zero-shot and fine-tuned models and devising several robust fine-tuning techniques. However, most existing methods rely on fully fine-tuning the entire model, which becomes increasingly impractical due to the substantial growth in model parameters. Consequently, fully fine-tuning pre-trained models for downstream tasks incurs significant computational, and memory overhead in training time and storage costs.
% \sy{need discuss switching other downstream task and most of the methods only focus classification.}
To address these problems, several approaches have been recently proposed that aim to fine-tune zero-shot models while preserving their robustness to OOD. These efforts include proposing diverse training strategies~\cite{flyp,lpft,maskfill} and ensembling the fine-tuned model with others~\cite{wiseft,modelsoup}, which have been shown to significantly enhance robustness compared to traditional fine-tuning.
However, most existing methods necessitate fine-tuning the entire model, which is becoming increasingly impractical with the exponential growth in model parameters. As a result, fully fine-tuning leads to significant computational and memory overheads during training, as well as increased storage costs. Moreover, the majority of these methods are limited to classification, thereby lacking their flexibility for other downstream tasks. These critical shortcomings highlight the need for new methods that \emph{maintain robustness while easily extending to a variety of new downstream tasks with efficiency}.
% These two shortcomings often lacking flexibility for application to different types of tasks. These two shortcomings highlight the need for new methods that \emph{maintain robustness while easily extending to a variety of new downstream tasks with efficient adaptation}.

A promising solution to this challenge is parameter-efficient transfer learning (PETL). This approach demonstrates effectiveness in addressing the challenges of catastrophic forgetting in continual learning~\cite{wang2022learning}. Nonetheless, such methods may exhibit a bias towards in-distribution (ID) data, resulting in the loss of the general knowledge of the pre-trained model, consequently reducing their generalization capacity to cope with distribution shifts~\cite{robusify}.

% Nonetheless, parameter-efficient techniques can be biased towards in-distribution (ID) data. The newly introduced parameters, lacking the generalized knowledge of the pre-trained model, can be easily biased to ID data, thereby diminishing the ability to handle distribution shifts~\cite{robusify}.

% In this paper, we focus on parameter-efficient learning techniques. On the surface, these methods hold great promise, especially in their potential to prevent catastrophic forgetting by introducing only a limited number of new parameters to adapt the pre-trained model. However, even well-known parameter-efficient learning methods tend to gradually introduce biases towards the in-distribution data and struggle to cope with distribution shifts~\cite{jain2023efficiently}.
In this paper, we introduce a novel efficient approach designed to enhance the robustness of fine-tuning: Parameter-Efficient Robust Fine-Tuning (\ours). Our method aims to fortify the OOD generalization capabilities of these large-scale models while simultaneously maintaining high ID accuracy and improving efficiency. With \ours, we freeze the pre-trained backbone model and introduce plug-and-play adapter modules without non-linear layers.  This design enables minimal parameter additions and also has no additional cost during inference through re-parametrization. \ours~leverages self-ensembling techniques, which have been demonstrated to enhance both accuracy and robustness~\cite{wiseft, modelsoup}. Specifically, we allow for dynamic model ensembling by stochastically dropping the adapter module and facilitating temporal ensembling through an exponential moving average. Most crucially, during evaluation, we re-scale the weights of the adapter and seamlessly integrate it within the pre-trained module via re-parametrization. We find this strategy enables effortless weight ensembling between the zero-shot and fine-tuned models.

% To preserve the viability of zero-shot inferences, we train both the image and text embedding models with deployed adapters in both the visual and text encoder blocks of CLIP. A straightforward training approach would be to train both encoders with the InfoNCE loss~\cite{Sohn_nips2016,oord2018representation} from CLIP, embracing the concept of ``finetuning like you pre-training''~\cite{flyp}. 
To preserve the viability of zero-shot inferences, we insert adapters in both the visual and text encoder blocks of CLIP. A simple training approach would be to train both encoders with the InfoNCE loss~\cite{Sohn_nips2016,oord2018representation} from CLIP.
However, this loss solely considers one-to-one correspondences and neglects multiple positive pairs in downstream task labels (e.g., samples of the same class labels in classification).  This oversight can distort representations by disregarding the pulling of positive samples while erroneously repelling them in the embedding space.
To tackle these challenges, we introduce a novel approach called MultiPos-NCE, which considers the characteristics of downstream task labels, particularly the presence of multiple positive samples. The proposed loss incorporates soft labels that distribute probabilities among these positive samples, encouraging their embeddings to pull close in the embedding space. Furthermore, we enhance the InfoNCE loss by introducing a margin for negative samples. This modification not only promotes the learning of highly discriminative features for downstream tasks but also protects against the unintentional repulsion of positive samples in the embedding space. 

% Consequently, as shown in the Fig.~\ref{}, \ours~ demonstrates a substantial enhancement in OOD performance, increasing it by X\%, while simultaneously reducing latency by X\% and preserving high ID accuracy.
% \sy{Sungyeon will describe last paragraph more.}
% Our method advances \textbf{parameter and memory efficiency}, which in turn \textbf{reduces the computational cost} of training time compared to traditional fine-tuning, meanwhile maintaining the \textbf{same inference time}. 
Our method advances \textbf{parameter} and \textbf{memory efficiency}, compared to traditional fine-tuning, meanwhile maintaining the \textbf{same inference time}. 
Crucially, our method exhibits \textbf{remarkable robustness}. To demonstrate the efficiency and effectiveness of our method, we first conduct an evaluation under various distribution shifts on ImageNet data for image classification. 
As shown in Fig.~\ref{fig:thumbnail}, by varying the four backbone networks, \ours~achieves higher OOD performance while using significantly fewer parameters and memory than the existing method with the same backbone.
% The results, as shown in the Fig.~\ref{fig:thumbnail}, \ours~ demonstrates a substantial enhancement in OOD performance, increasing it by 1.5\%p, while simultaneously reducing latency by X\% and preserving high ID accuracy.
Furthermore, in few-shot learning scenarios, \ours~surpasses existing approaches by a clear margin, achieving enhanced robustness with fewer parameters. 

Beyond these achievements, we recognize the current focus of robust fine-tuning tends to be limited to classification tasks, prompting us to extend the utility of our method. Thanks to its plug-and-play design, our approach can be effortlessly adapted to \textbf{a variety of tasks}. Its effectiveness is further demonstrated in cross-modal retrieval tasks, where it surpasses existing robust fine-tuning methods. Moreover, we show our method can serve as an effective training strategy for open-vocabulary segmentation tasks, underscoring its versatility and broad applicability.

% To rectify this, we leverage soft labels, which accommodate multiple positive samples in contrast to standard one-hot labels. Specifically, we spread the probabilities across multiple positive samples, ensuring their embeddings are pulled closer together. Additionally, label smoothing can be applied by a weighted sum of this soft label with uniform distribution to harness its advantages. Furthermore, we modify the InfoNCE loss function to include a negative margin for each positive sample. This boosts the learning of highly discriminative representations for downstream tasks and also mitigates that positive samples are not mistakenly repelled.




==> Sections/_1_introduction_backup.tex <==
\section{Introduction}
\label{sec:intro}



% \begin{wrapfigure}{r}{0.4\textwidth}
% \vspace{-15mm}
% \begin{center}
% \includegraphics[width = 0.4\textwidth]{figs/Figure_thumbnail2.pdf}
% \end{center}
% \vspace{-6mm}
% \caption{
% Comparative analysis of performance versus memory usage among robust fine-tuning methods. Memory usage is measured on an NVIDIA 3090 GPU at a batch size of 16. Our method utilizes less memory, which supports easily scaling up to larger models and broader applications, unlike most other methods.} 
% \label{fig:thumbnail}
% \vspace{-8mm}
% \end{wrapfigure}
\iffalse
The emergence of large-scale models pre-trained jointly on image and text data, such as CLIP~\cite{clip}, brings a paradigm shift in the field of computer vision. The models leverage the power of contrastive learning to align vast collections of image-text pairs sourced from the web, enabling them to capture intricate relations between these two modalities. This training enables them to perform zero-shot classification, where previously unseen images are classified by comparing their embeddings with textual class descriptions. Impressively, these models show notable zero-shot performance across a wide range of data distributions.

While their performance is impressive in a zero-shot context, it still does not measure up to supervised models.
To unlock their full potential for downstream tasks, fine-tuning is often necessary. This boosts their performance significantly on the target distribution. Yet, a notable challenge emerges: traditional fine-tuning diminishes their capacity to generalize to out-of-distribution (OOD) data~\cite{clip, scalingshifting, pham2023combined, lpft}. This decrease in adaptability raises concerns, especially when deploying these models in the real world with unpredictable data variances. 
To address these problems, several approaches have been recently proposed that aim to fine-tune zero-shot models while preserving their robustness to OOD~\cite{flyp,lpft,maskfill, wiseft,modelsoup}. 
However, most existing methods necessitate fine-tuning the entire model, which becomes impractical as model sizes grow, resulting in high computational cost, memory, and storage demands. 
Moreover, the majority of these methods are limited to classification, thereby lacking their flexibility for other downstream tasks. These critical shortcomings highlight the need for new methods that {maintain robustness while easily extending to a variety of new downstream tasks with efficiency}.

\begin{figure} [!t]
\centering
\includegraphics[width = 0.6\linewidth]{figs/Figure_thumbnail2.pdf}
\vspace{-3mm}
\caption{Comparative analysis of performance versus memory usage among robust fine-tuning methods. Memory usage is measured on an NVIDIA 3090 GPU at a batch size of 16. Our method utilizes less memory, which supports easily scaling up to larger models and broader applications, unlike most other methods.} 
\label{fig:thumbnail}
\vspace{-6mm}
\end{figure}



% A promising solution to this challenge is parameter-efficient transfer learning (PETL). This approach demonstrates effectiveness in addressing the challenges of catastrophic forgetting in continual learning~\cite{wang2022learning}. Nonetheless, such methods may exhibit a bias towards in-distribution (ID) data, resulting in the loss of the general knowledge of the pre-trained model, consequently reducing their generalization capacity to cope with distribution shifts~\cite{robusify}.


In this paper, we introduce a novel efficient approach designed to enhance the robustness of fine-tuning: Parameter-Efficient Robust Fine-Tuning (\ours). Our method aims to fortify the OOD generalization capabilities of these large-scale models while improving both high in-distribution accuracy and efficiency. With \ours, we freeze the pre-trained backbone model and introduce plug-and-play adapter modules without non-linear layers.  This design enables minimal parameter additions and also has no additional cost during inference through re-parametrization.
However, even with minimal parameter additions in PERFT, there still remains a risk of distribution shifts~\cite{robusify}. To address this, \ours~employs novel self-ensembling techniques to prevent forgetting the knowledge of the pre-trained model. 
% which have been shown to enhance both accuracy and robustness~\cite{wiseft, modelsoup}. 
Specifically, we enable dynamic ensembling by stochastically dropping the module and temporal ensembling through an exponential moving average. Moreover, during evaluation, we re-scale the weights of the adapter and integrate it into the pre-trained layer via re-parametrization, which enables effortless weight ensembling between the zero-shot and fine-tuned models.
\fi
\sy{In pursuit of a solution that meets these criteria, we draw inspiration from recent advances in Parameter-Efficient Transfer Learning (PETL), a new transfer learning technique updates only a minimal subset of parameters while keeping the bulk of the pre-trained parameters frozen. This approach not only enables parameter efficiency but also facilitates rapid adaptation to new tasks without the risk of catastrophic forgetting, often resulting in enhanced robustness during OOD evaluations. However, as indicated in our findings, these methods still fall short of achieving the OOD performance levels of existing robust fine-tuning techniques by a significant margin.

This paper introduces a novel approach that significantly boosts the OOD generalization capabilities of PETL methods. We present the "Robust Adapter", an adapter module that employs self-ensembling techniques to preserve the generalizable knowledge inherent in the pre-trained zero-shot model. Our key innovation lies in the strategic integration of adapted modules with less-adapted parameters within the model, achieving a compromising solution that balances both specific downstream tasks and generalizability goals. Specifically, this is first achieved through random dropping of adapter modules, implicitly dynamic ensembling subnetworks comprising both pre-trained layers and adapter modules. Additionally, we leverage a momentum update strategy to accumulate parameters that are being adapted over time, facilitating a temporal ensemble that bridges less-adapted and adapted parameters. Furthermore, during evaluation, we re-scale the weights of the adapter and integrate it into the pre-trained layer via re-parametrization, which enables effortless weight ensembling between the pre-trained and fine-tuned models without two entire models.}

% \sy{To ensure task versatility by enabling zero-shot inferences, we insert adapters in both the visual and text encoder blocks of CLIP.}
To achieve versatility across various tasks through zero-shot inferences, we aim to fine-tune the joint embedding space of both visual and text modalities by inserting adapters into both encoders in CLIP.
A basic training approach would be to train both encoders with the InfoNCE loss~\cite{Sohn_nips2016,oord2018representation} from CLIP.
However, this loss solely considers one-to-one correspondences and neglects multiple positive pairs in downstream task labels (e.g., samples of the same class labels in classification).  This oversight can distort representations by disregarding the pulling of positive samples while erroneously repelling them in the embedding space.
To tackle these challenges, we introduce a novel approach called MultiPos-NCE, which considers the characteristics of downstream task labels, particularly the presence of multiple positive samples. Our loss employs soft labels that distribute probabilities among these positive samples, encouraging their embeddings to pull close in the embedding space. Furthermore, we enhance the InfoNCE loss by introducing a margin for negative samples. This modification not only promotes the learning of highly discriminative features for the tasks but also protects against the unintentional repulsion of positive samples in the embedding space. 

Our method advances \textbf{parameter} and \textbf{memory efficiency}, compared to traditional fine-tuning, meanwhile maintaining the \textbf{same inference time}. 
Crucially, our method exhibits \textbf{remarkable robustness}. To demonstrate the efficiency and effectiveness of our method, we first conduct an evaluation under various distribution shifts on ImageNet data for image classification. 
As shown in Fig.~\ref{fig:thumbnail}, \ours~achieves higher OOD performance while using significantly fewer parameters and memory than the existing methods with the same backbone.
In few-shot learning scenarios, our method also surpasses existing approaches by a clear margin, achieving enhanced robustness with fewer parameters. 
\iffalse
% Beyond these achievements, we recognize the current focus of robust fine-tuning tends to be limited to classification tasks, prompting us to extend the utility of our method. Thanks to its plug-and-play design, our approach can be effortlessly adapted to \textbf{a variety of tasks}. Its effectiveness is further demonstrated in cross-modal retrieval tasks, where it surpasses existing robust fine-tuning methods. Moreover, we show our method can serve as an effective training strategy for open-vocabulary segmentation tasks, underscoring its versatility and broad applicability.
% Beyond these achievements, we recognize the current focus of robust fine-tuning tends to be limited to classification tasks, prompting us to extend the utility of our method. 
\fi
Moreover, thanks to the plug-and-play design of ~\ours, it can be effortlessly adapted to \textbf{a variety of tasks}. Its effectiveness is further demonstrated in cross-modal retrieval, outperforming existing robust fine-tuning methods. Finally, it proves to be a superior training strategy for open-vocabulary segmentation, underscoring its versatility and broad applicability.

==> Sections/_4_experiments_backup.tex <==


\section{Experiments}
\label{sec:experiments}


We demonstrate the robustness of \ours~against distribution shits and its efficiency on the four downstream tasks such as image classification (Sec.~\ref{sec:classification}), few-shot image classification (Sec.~\ref{sec:fewshot}), cross-modal retrieval, and open-vocabulary segmentation (Sec.~\ref{sec:downstream}). 
Finally, we examine the impact of proposed components and hyperparameters (Sec.~\ref{sec:ablation}).
% by conducting thorough ablation studies.


\subsection{Datasets}\label{sec:datasets}
% \noindent{\textbf{Image Classification.}} We use ImageNet (IN)~\cite{Imagenet} as the ID dataset for fine-tuning; we evaluate the robustness of the models on five standard OOD datasets that represent five different types of OOD scenarios:
% ImageNetV2 (IN-V2)~\cite{recht2019imagenet} is a new test set for ImageNet with distribution shift.
% ImageNet-R (IN-R)~\cite{hendrycks2021many} consists of various artistic renditions (\eg, painting, cartoons) of 200 ImageNet classes
% ImageNet-Sketch (IN-Sketch)~\cite{wang2019learning} contains sketch images of 1000 ImageNet classes. 
% ObjectNet~\cite{barbu2019objectnet} is a test set that contains images with 313 object classes collected from new viewpoints on new backgrounds, where 113 classes overlap with ImageNet. 
% ImageNet-A (IN-A)~\cite{hendrycks2021natural} consists of natural images that are misclassified by a pre-trained ResNet-50~\cite{resnet} for 200 ImageNet classes.
% Note that these datasets except ObjectNet are also used for few-shot image classification, where we follow the few-shot setting in~\cite{clip}.
The details of all datasets are elaborated in the appendix.




\noindent{\textbf{Image Classification.}}
We use ImageNet (IN)~\cite{Imagenet} as the ID dataset for fine-tuning; we evaluate the robustness of the models on five standard OOD datasets with different distribution shifts, following prior work~\cite{wiseft,flyp,maskfill,clip,lpft}: ImageNetV2 (IN-V2)~\cite{recht2019imagenet}, 
ImageNet-R (IN-R)~\cite{hendrycks2021many}, ImageNet-Sketch (IN-Sketch)~\cite{wang2019learning}, ObjectNet~\cite{barbu2019objectnet}, and ImageNet-A (IN-A)~\cite{hendrycks2021natural}. Note that these datasets except ObjectNet are also used in a few-shot setting following previous work~\cite{cocoop, coop, repadapter,clipood}.

\noindent{\textbf{Cross-Modal Retrieval.}}
We utilize two standard benchmarks for image-text cross-modal retrieval, COCO~\cite{Mscoco} as ID and Flickr30K~\cite{Flickr30k_b} as OOD. For these two datasets, each image is associated with the corresponding five captions.
% Specifically, COCO is exploited as the ID dataset, and Flickr30K is utilized as ㄱthe OOD dataset which has distribution shifts in both image and text modalities. 
% In COCO, there are 123,287 images, and we follow the data split of~\cite{karpathy2015deep} with 113,287 images for training, and 5,000 images for testing.
% Flickr30K contains 29,000 images for training and 1,000 images for testing.

\noindent{\textbf{Open-Vocabulary Segmentation.}}
% By following~\cite{ovseg}, we train the models on COCO Captions~\cite{chen2015microsoft} and evaluate them on ADE20K~\cite{zhou2019semantic}, Pascal Context~\cite{mottaghi2014role}, and Pascal VOC~\cite{Pascalvoc} with 20 categories (PAS-20).
% Specifically, we exploit ADE20K in two versions, one with 150 frequently used categories (A-150) and the other with diverse 847 categories (A-847).
% % Moreover, we also utilize Pascal Context in two versions, one with 59 frequently used categories (PC-59) and the other with the whole 459 categories (PC-459).
% We use two versions of Pascal Context, one with 59 frequently used categories (PC-59) and the other with the whole 459 categories (PC-459).
Following our baseline method~\cite{ovseg}, we train a CLIP model on the COCO Captions dataset \cite{chen2015microsoft} and test them on several benchmarks as OOD: ADE20K \cite{zhou2019semantic}, Pascal Context \cite{mottaghi2014role}, and Pascal VOC \cite{Pascalvoc}. 
We evaluate ADE20K in A-150 and A-847, and Pascal Context in PC-59 and PC-459 category versions.
% We consider two sets of categories for ADE20K (150 and 847 categories) and for Pascal Context (59 and 459 categories).




\subsection{Implementation Details}\label{sec:details}
\noindent{\textbf{Network Architectures.}}
We adopt the pre-trained CLIP models from OpenAI~\cite{clip} with four different sizes of image encoder, ViT-B/32, ViT-B/16, ViT-L/14, and ViT-L/14@336px~\cite{ViT}.
% Unless otherwise specified, we use the CLIP ViT-B/32 model by default.

\noindent{\textbf{Network Optimization.}}
% \bs{Details of optimizer would be revised}
% For all experiments, our model is trained using AdamW without weight decay for 10 epochs with a batch size of 512.
For all experiments, our model is trained using AdamW without weight decay for 10 epochs with a batch size of 512, except for open-vocabulary  segmentation, which is trained for 5 epochs following previous work~\cite{ovseg}.
The initial learning rate is set to $\expnum{5}{4}$, using a cosine scheduling with 500 warm-up steps.
% For the classification task, we follow the setting presented in~\cite{flyp}, and more details can be found in the appendix.
We follow the settings in~\cite{flyp} for full-shot classification,~\cite{clipood} for few-shot classification, and~\cite{ovseg} for open-vocabulary segmentation. More details are in the appendix.
% Note that all parameters in CLIP image and text encoders are fixed during training.
% Following previous work~\cite{wiseft, flyp, clip, maskfill}, we do not employ extra image augmentation except for resizing and cropping.
% For full~/~few-shot classification task, we use the text prompt template as used in CLIP~\cite{clip}.
% More details on open-vocabulary segmentation are described in our appendix.

% \input{tabs/table_PETL.tex}


\noindent{\textbf{Hyperparameters.}}
The drop probability $p$ is set to 0.2.
The momentum update rate $m$ in Eq.~\ref{eq:Accumulation} is set to 0.999.
The margin $\delta$ in Eq.~\ref{eq:MultiPos-NCE} is 0.05.
For classification tasks, following the WiSE-FT~\cite{wiseft}, we use the re-scaling coefficient $\alpha$ in Eq.~\ref{eq:rescale} of 0.5. For cross-modal retrieval and open-vocabulary segmentation tasks, we set $\alpha$ to its optimal values of 0.8 and 0.4, respectively.
We set the smoothing coefficient $\epsilon$ in Eq.~\ref{eq:soft_label} to 0.05 for classification, and 0 for other tasks.
% Unless otherwise specified, we fix these hyper-parameters for all experiments.

% \noindent{\textbf{Evaluation Metrics.}}
% We exploit {top-1 accuracy} for image classification, {recall at K} (R@K=1, 5, 10) for cross-modal retrieval, and {mIoU} for open-vocabulary segmentation as evaluation metrics.


\input{tabs/table1.tex}




\subsection{Results} 
% We evaluate the robustness of our models against distribution shifts on full~/~few-shot image classification.
% Moreover, we extend the parameter-efficient robust fine-tuning scenario to diverse tasks, such as cross-modal retrieval and open-vocabulary segmentation.

\subsubsection{ImageNet Classification.}\label{sec:classification}

We compare \ours~with zero-shot, conventional fine-tuning approach, and previous robust fine-tuning methods, WiSE-FT~\cite{wiseft}, LP-FT~\cite{lpft}, Model Soup~\cite{modelsoup}, FLYP~\cite{flyp}, and Mask-Fill~\cite{maskfill} on the in-distribution (ID) dataset and five out-of-distribution (OOD) datasets.
% For a fair comparison, we adopt ViT-B/32, ViT-B/16, and ViT-L/14@336px as the image encoder.
We report the performance of WiSE-FT with the default mixing coefficient of 0.5. We take the \textit{uniform soup} as the default method of~\cite{modelsoup}.
% , which shows the best OOD performance among Model Soup variants~\cite{modelsoup}.
% Table~\ref{tab:comparison_finetuned} shows the comparison of our method with the previous arts on OOD datasets and the number of trainable parameters. 
The results and the number of trainable parameters are summarized in Table~\ref{tab:comparison_finetuned}.
Specifically, our method improves the previous state of the art by a significant margin as 1.2\%p and 1.5\%p in terms of OOD avg. with CLIP ViT-B/32 and CLIP ViT-B/16, respectively; even though our method only requires much less tunable parameters (20.5M) than the others ($>$80M).
Moreover, our method scales efficiently yet effectively to the CLIP ViT-L/14@336px model, showing a notable 2\%p improvement in OOD performance over WiSE-FT. 
While the Uniform Soup achieves superior results on IN and IN-V2, it involves a complex ensemble of finely tuned models, leading to increased computational and training resource demands. In contrast, our method offers a more cost-efficient approach to enhancing robustness, as evidenced by the pronounced gains observed in the most distribution-shifted datasets, IN-A and IN-R. 

% Moreover, we also compare the zero-shot classification which is directly evaluated with the pre-trained CLIP model, and the conventional fine-tuning which is tuned on each evaluation dataset.
% The fine-tuned model outperforms the zero-shot classification in terms of ID accuracy, while it underperforms the zero-shot classification in terms of OOD accuracy due to the diminished generalization to OOD, as shown in Table~\ref{tab:comparison_finetuned}.
% It implies that robust fine-tuning is essential to the real-world scenario.

% Table~\ref{tab:comparison_finetuned} shows that our method outperforms the previous arts in terms of the average of OOD top-1 accuracy (OOD avg.).
% Specifically, our method improves the previous state of the art by a significant margin as 1.2\%p and 1.5\%p in terms of OOD avg. with CLIP ViT-B/32 and CLIP ViT-B/16, respectively; even though our method only requires much less tunable parameters (20.5M) than the others ($>$80M).
% Moreover, thanks to the re-parametrization, our method has the same time costs for inference as the weight-space ensemble methods.
% These properties of our method allow it to serve as an efficient plug-and-play module with small parameter requirements.
% Although Uniform Soup~\cite{modelsoup} achieves the best performance on IN and IN-V2, it is worth noting that it exploits a large number of fine-tuned models with various hyperparameters and thus it is inefficient to the training costs. 





% \input{tabs/table3.tex}


\input{tabs/table2.tex}

\subsubsection{Few-Shot ImageNet Classification.}\label{sec:fewshot}
We further investigate whether our model is robust even when access to the images used for training is limited.
To this end, we evaluate our models on the ID dataset and OOD datasets for few-shot classification, especially 16-shot.
We compare ours with the previous methods for parameter-efficient tuning~\cite{coop, cocoop, repadapter} and robust fine-tuning~\cite{clipood}. 
We also examine the effectiveness of our model by utilizing the low-rank adapter instead of the full-rank one, where the number of trainable parameters of the low-rank adapter is as small as CoCoOp~\cite{cocoop} and RepAdapter~\cite{repadapter}.
% We adopt CLIP ViT-B/16 as the visual backbone.
% and exclude ObjectNet~\cite{barbu2019objectnet} for a fair comparison.
We report the results in Table~\ref{tab:fewshot}.
Compared to the state of the art~\cite{clipood}, our method improves the performance on all evaluation datasets, even though our model requires four times fewer trainable parameters. %than it.
Moreover, our model with the rank-1 adapter beats CoOp and CoCoOp by a large margin of 2.3\%p and 1.7\%p in terms of the average OOD top-1 accuracy, while the number of tunable parameters is comparable.
It implies that our method allows it to retain the generalization capability on the OOD datasets with extremely small parameters while keeping the ID accuracy.



\subsection{Broader Downstream Tasks.}\label{sec:downstream}
Beyond classification tasks, we broaden the scope to robustly fine-tune diverse downstream tasks, such as cross-modal retrieval and open-vocabulary segmentation.

\input{tabs/table3.tex}





\noindent{\textbf{Cross-Modal Retrieval.}}
We evaluate our model on COCO~\cite{Mscoco} and Flickr30K~\cite{Flickr30k_b} for cross-modal retrieval, where the model is only fine-tuned on the COCO dataset.
Since most previous methods for robust fine-tuning are limited to the classification task only, we compare our method with FLYP~\cite{flyp} from our re-implementation.
We further compare ours with supervised specialists~\cite{li2020unicoder, chen2020uniter, gan2020large, li2020oscar, yu2021ernie}.
As shown in Table~\ref{tab:Retrieval}, our method outperforms FLYP in terms of all evaluation metrics except R@10 for text retrieval on Flickr30K.
Moreover, our method using CLIP ViT-L/14 surpasses the supervised specialists that have a similar size and are trained on both datasets, respectively.
Note that even though we do not utilize Flickr30K in training at all, it outperforms supervised methods.


\input{tabs/table4.tex}
\input{tabs/table_comp_abl.tex}

\noindent{\textbf{Open-Vocabulary Segmentation.}}
% We build a model for open-vocabulary segmentation upon OVSeg~\cite{ovseg}.
We show that using our method for the fine-tuning stage of the CLIP model within the OVSeg framework enhances open-vocabulary segmentation performance.
Specifically, we equip the full-rank adapters in both the CLIP image and text encoders of OVSeg and fine-tune them while the pre-trained encoders are frozen.
By following~\cite{ovseg}, we adopt Swin-B~\cite{liu2021swin} as a backbone for a mask proposal network which is trained on the COCO-Stuff~\cite{caesar2018coco} dataset.
% The model is trained on COCO Captions~\cite{chen2015microsoft} and evaluated on five datasets that do not share semantic categories with the training dataset, as shown in Table~\ref{tab:ovseg}.
The open-vocabulary classification model using CLIP ViT-L/14 is trained on masked images from COCO Captions~\cite{chen2015microsoft} and evaluated on five unseen datasets, as shown in Table~\ref{tab:ovseg}.
% The performance of zero-shot segmentation on these datasets is presented in Table~\ref{tab:ovseg}. 
% \dk{It should be noted that OVSeg is trained using a contrastive loss akin to FYLP. WiSE-FT and Mask-Fill cannot be directly applicable to this task as their classifiers work only for ImageNet classes.}
% We note that the original fine-tuning of OVSeg model leverages a contrastive loss akin to the FYLP~\cite{flyp} while freezing the text encoder.
Compared with the original OVSeg fine-tuning, 
where first stage is similar to FLYP~\cite{flyp} while freezing the text encoder,
our approach yields a significant increase in performance, with mIoU improvements of 1.3\%p, 0.2\%p, 3.3\%p, and 1.9\%p on the A-847, PC-459, PC-59, and PAS-20, respectively.
These results confirm that our method enhances the robustness of unseen classes, demonstrating it to be a promising approach for the open-vocabulary segmentation task.
% Meanwhile, our method demonstrates performance comparable to OVSeg on A-150.

% The experimental results of our method on the two downstream tasks suggest that our method can be equipped with arbitrary CLIP-based models for diverse downstream tasks while requiring only a few memory and computational costs for training and no additional cost for inference. 
\input{tabs/table_ablation.tex}

\subsection{Ablation Studies}
\label{sec:ablation}
% We investigate the impact of the proposed components and hyperparameters on the classification performance of our method.
% We adopt CLIP ViT-B/32 as a visual backbone and measure the performance on the ID dataset and the five OOD datasets.
% The results of the ablation studies are presented in Table~\ref{tab:ablation}.%, where the \colorbox{grey}{grey box} denotes our method.





\noindent{\textbf{Impact of Each Component.}}
% The components of our method include stochastic dropping, momentum update, re-scaling in inference, and MultiPos-NCE loss.
% We investigate the impact of each component in our method.
% To this end, we evaluate models by discarding each component from \colorbox{grey}{Ours}, which is summarized in Table~\ref{tab:component}.
We investigate the impact of each component by discarding each component, which is summarized in Table~\ref{tab:ablation_components}.
Both stochastic dropping and momentum update improve the OOD accuracy while keeping the ID performance as the dynamic and temporal ensembles allow to retain the robustness of the pre-trained models.
Meanwhile, MultiPos-NCE loss improves both ID and OOD accuracy since the original InfoNCE loss ignores the multiple positive relations within the label space.
% Moreover, the re-scaling strategy improves the OOD performance greatly since it controls the balance between the model trained on the ID dataset and the pre-trained model with generalization capacity to OOD.
Re-scaling is particularly effective for OOD performance since it controls the balance between zero-shot and fine-tuned states.
% Finally, adopting only pure adapters without all components markedly undermines OOD accuracy even worse than zero-shot performance.
% It implies that all our components for \ours~are crucial to fortify the generalization capacity.
Omitting all components results in significantly reduced OOD accuracy, suggesting the integral role of each element in fortifying generalization.


\begin{wrapfigure}{r}{0.5\textwidth}
\vspace{-3mm}
\begin{center}
\includegraphics[width = 0.5\textwidth]{figs/alpha_ablation.pdf}
\end{center}
\vspace{-6mm}
\caption{
Performance of our method varying re-scaling coefficient $\alpha $ against WiSE-FT.} 
\label{fig:rescaling}
\vspace{-8mm}
\end{wrapfigure}

\noindent{\textbf{Hyperparameters and Loss Variations.}} We investigate the impact of hyperparameters including the drop probability $p$ in Eq.~\ref{eq:Stochastic}, the momentum update rate $m$ in Eq.~\ref{eq:Accumulation} and the margin of our loss $\delta$ in Eq.~\ref{eq:MultiPos-NCE}. 
Table~\ref{tab:ablation_hyperparams} shows gradual performance gains with margin $\delta$ up to 0.05. Removing soft labeling while using only margin notably reduces OOD performance. As shown in Table~\ref{tab:stochastic} and~\ref{tab:ema}, each hyperparameter brings enhanced performance improvement compared to when it is set to 0, regardless of specific values; hence, we do not effort to find the best hyperparameters. Fig.~\ref{fig:rescaling} shows the impact of varying the re-scaling coefficient $\alpha$ in Eq.~\ref{eq:rescale}. Compared to WiSE-FT~\cite{wiseft}, our method shows less sensitivity to changes in $\alpha$, sustaining superior performance across various settings, not limited to the default.

% \begin{figure}[!h]
%     \centering
%     {\includegraphics[width = 0.5\linewidth]{figs/alpha_ablation.pdf}}
%     \vspace{-2mm}
%     \caption{Performance of our method varying re-scaling coefficient $\alpha $ against WiSE-FT.}
%     \label{fig:rescaling}
%     \vspace{-4mm}
% \end{figure}




==> tabs/table_PETL.tex <==
\begin{table}[!t]
\caption{Top-1 accuracy of PETL methods on ImageNet (ID) and OOD datasets with ViT-B/32. Superscripts denote adapter rank.
}
\vspace{-2mm}
\fontsize{7}{9.3}\selectfont
\setlength{\tabcolsep}{2pt}
\centering
\begin{tabularx}{1.0\textwidth}
    {
      p{0.182\textwidth}
      >{\centering\arraybackslash}p{0.15\textwidth}
      >{\centering\arraybackslash}p{0.065\textwidth}
      >{\centering\arraybackslash}p{0.065\textwidth}
      >{\centering\arraybackslash}p{0.065\textwidth}
      >{\centering\arraybackslash}p{0.1\textwidth}
      >{\centering\arraybackslash}p{0.1\textwidth}
      >{\centering\arraybackslash}p{0.065\textwidth} |
      >{\centering\arraybackslash}p{0.11\textwidth}
      }
     \toprule
    {\multirow{1}{*}[-4.5mm]{\textbf{Methods}}}& \multirow{1}{*}[-0.5mm]{\textbf{Trainable}}&
    \multicolumn{1}{c}{\textbf{ID}} & \multicolumn{6}{c}{\textbf{Out-Of-Distribution~(OOD)}} \\ [-0.3ex]  \cmidrule(lr){3-3}  
    \cmidrule(lr){4-9} &\multirow{1}{*}[0.5mm]{\textbf{Params (M)}} & IN & IN-V2 & IN-R&  {IN-Sketch} &{ObjectNet}& IN-A & {OOD avg.} \\  [-0.4ex] \midrule
     AdaptFormer$^\textrm{16}$~\cite{adaptformer} & 0.5 & \textbf{74.7}& 64.3 & 63.8 &41.7 & 45.5 & 29.3 & 48.9\\ 
     RepAdapter$^\textrm{16}$~\cite{repadapter} & 1.0 &  74.3 & 64.4& 65.1& 42.4& 46.0& 30.4 & 49.7 \\
       Ours$^\textrm{16}$ & 1.0 &    {74.5}&  \textbf{65.1} &  \textbf{69.5} &  \textbf{45.8} &   \textbf{47.9} &  \textbf{34.0}&  \textbf{52.5} \\ 
     \midrule
    \vspace{-2.5mm}
     AdaptFormer$^\textrm{128}$~\cite{adaptformer} &3.9 &  75.6 & 64.5 & 61.7 & 41.0 & 45.0 & 29.3 & 48.3 \\ 
     RepAdapter$^\textrm{128}$~\cite{repadapter} &7.8&   \textrm{76.3} & 65.2 & 62.7& 41.9& 45.7& 29.2& 48.9 \\
       Ours$^\textrm{128}$ & 7.8 &  \textbf{76.7} &   \textbf{66.9} &  \textbf{70.2} &  \textbf{47.1} &   \textbf{48.7} &  \textbf{35.5} &  \textbf{53.7} \\  \midrule
    \vspace{-2.5mm}
     AdaptFormer$^\textrm{Full}$~\cite{adaptformer} & 20.5 & 77.2 & 66.4 & 60.6 & 42.2 & 45.2& 28.0& 48.5 \\
     RepAdapter$^\textrm{Full}$~\cite{repadapter} & 20.5 &  76.9 & 65.5& 60.1& 41.3& 44.2& 27.6& 47.7 \\
       Ours$^\textrm{Full}$ &  20.5 & \textbf{77.7}  &  \textbf{67.7} & \textbf{70.8} &    \textbf{47.8}   &  \textbf{49.7} &  \textbf{35.6}  &  \textbf{54.3} \\ \bottomrule 
\end{tabularx}
\vspace{-3.5mm}
\label{tab:petl_comparison}
\end{table}

